From CNNs to Transformers in Multimodal Human Action Recognition: A Survey

Due to its widespread applications, human action recognition is one of the most widely studied research problems in Computer Vision. Recent studies have shown that addressing it using multimodal data leads to superior performance as compared to relying on a single data modality. During the adoption of deep learning for visual modelling in the last decade, action recognition approaches have mainly relied on Convolutional Neural Networks (CNNs). However, the recent rise of Transformers in visual modelling is now also causing a paradigm shift for the action recognition task. This survey captures this transition while focusing on Multimodal Human Action Recognition (MHAR). Unique to the induction of multimodal computational models is the process of "fusing" the features of the individual data modalities. Hence, we specifically focus on the fusion design aspects of the MHAR approaches. We analyze the classic and emerging techniques in this regard, while also highlighting the popular trends in the adaption of CNN and Transformer building blocks for the overall problem. In particular, we emphasize on recent design choices that have led to more efficient MHAR models. Unlike existing reviews, which discuss Human Action Recognition from a broad perspective, this survey is specifically aimed at pushing the boundaries of MHAR research by identifying promising architectural and fusion design choices to train practicable models. We also provide an outlook of the multimodal datasets from their scale and evaluation viewpoint. Finally, building on the reviewed literature, we discuss the challenges and future avenues for MHAR.

==> extra.tex <==
The Transformer \cite{vaswani2017attention} was first proposed as a remedy to some limitations of sequence modeling architectures, originally designed to deal with whole sequences at once, which allows parallelization of some operations (as opposed to RNNs, which are sequential in nature), and reduces the locality bias of traditional networks (such as CNNs). \par

\textbf{Self-attention (SA).} SA is the core component of the Transformer, receiving the input representation $X \in \mathbb{R}^{T^{(X)}\times d_m} $ and a memory $M \in \mathbb{R}^{T^{(X)}\times d_m}$, where $T^{( \cdot)}$ is the sequence length and $d_m$ is the dimensionality of each element in the sequence (namely tokens). In practice, $X = M$, hence the name self-attention. But this may be not necessarily the case, and when $X \neq M$, the same operation is denoted as cross attention (CA). This type of attention has already been shown in \cite{vaswani2017attention}, when the decoder attends to the encoder representation and, in general, it provides a way to incorporate external information M. In each Transformer layer, $X$ is mapped to a set of queries $Q \in \mathbb{R}^{T^{(X)}\times d_k}$ , while $M$ is mapped to a set of paired keys $K \in \mathbb{R}^{T^{(X)}\times d_k}$ and values $V \in \mathbb{R}^{T^{(X)}\times d_k}$ ,
where $d_k = d_m/h$ and $h$ is the number of heads (defined below). \par

The Transformer implements the relationship between different elements through a non-local operation, where the level of connection is determined by computing the dot-product between $Q$ and $K$. The resulting matrix is utilized to determine the contribution of each value to the output representation of all other values. Intuitively, this dot-product establishes the relevance that each value has for a given query, and weighs the interactions among values accordingly. More formally:

\begin{equation}
    Att(Q, K, V) = softmax (\frac{QK^T}{\sqrt{d_k}})V.
\end{equation}

\textbf{Transformer Layer.} A complete Transformer layer is composed of two or more sub-layers, followed by a residual connection and layer normalization \cite{ba2016layer} (see Fig. \ref{fig:transformer}). More formally, the output of each sub-layer, which is fed as input to the next, is defined as $LayerNorm(X + Sublayer(X))$. $Sublayer(X)$ is the function implemented by the sub-layer
itself: either Multi-Head Attention (MHA) or position-wise Feed-Forward Network (FFN)  which we define below. \par

Similar to the multiple filters in a convolutional layer, MHA has been proposed in \cite{vaswani2017attention}, where $X$ and $M$ were mapped to h different representation sub-spaces (i.e., different sets of $Q$, $K$ and $V$) in order to perform different attention operations simultaneously. The output of each head is concatenated and mapped back to a common $d_m$-dimensional space through a linear transformation $W^{(O)} \in \mathbb{R}^{(d_k) \times d_m}$:

\begin{equation}
        MHA(X,M) = Concat(head_1,..., head_h)W^{(O)}  
\end{equation}
where
\begin{equation}
head_i = Att(XW^{(Q)}_i,MW^{(K)}_i ,MW^{(V)}_i),       
\end{equation}
 

\noindent and $W^{(\cdot)}_i \in \mathbb{R}^{d_m \times d_k}$. Note that each sub-layer will have different weights $W$, we omit these for simplicity. \par
While it has been shown that the non-local mixing of
tokens (which happens in the SA operation) is the key for the success of many recent models (e.g., \cite{ilya2021mlp} and \cite{lee2021fnet}), including the Transformer, this is not enough to build a successful model \cite{dong2021pure}.  \par

\begin{figure}
    \centering
    \includegraphics[height=0.5\textwidth,width=0.6\textwidth]{images/transformer.png}
    \caption{The Transformer, as originally proposed in \cite{vaswani2017attention}, depicted through visualization \cite{selvasurvey2022videotrans}.}
    \label{fig:transformer}
\end{figure}

\textbf{Masked Self-attention.} The SA operation can optionally use a mask to ignore certain tokens. This idea has already introduced in \cite{vaswani2017attention} for the masked SA sub-layer in the decoder, been so that tokens not yet predicted could not be attended. Provided that in SA $M = X$, the result of the dot product $QK^T \in \mathbb{R}^{T^{(X)}\times T^{(X)}}$ is a square matrix. The mask is then defined as $M = (m_{ij} ), 1 \leq i, j \leq T^{(X)}$ and set $m_{ij} = {-}\infty \leftrightarrow i < j$ and $m_{ij} = 0$ otherwise. The mask is then added to the result of the normalized dot-product in Eq. (1), just before the softmax. In this way, the exponential function in the softmax draws the attention values for the masked attention pairs to 0, ignoring their contribution to $V$.

\textbf{Positional Encodings (PE).} The SA operation and, by extension, Transformers are permutation-invariant. In order to incorporate structural biases in the attention computation, \cite{vaswani2017attention} proposes adding absolute positional encodings to the input sequence $X$, prior to SA. The encodings $E \in \mathbb{R}^{T^{(X)}\times d_m}$, apart from absolute, are fixed as its elements are defined using a set of sinusoidal functions (also known as Fourier features, see \cite{vaswani2017attention} for details).
